Solution and Fitness Evolution (SAFE): Coevolving Solutions and Their Objective Functions

We recently highlighted a fundamental problem recognized to confound algorithmic optimization, namely, \textit{conflating} the objective with the objective function. Even when the former is well defined, the latter may not be obvious, e.g., in learning a strategy to navigate a maze to find a goal (objective), an effective objective function to \textit{evaluate} strategies may not be a simple function of the distance to the objective. We proposed to automate the means by which a good objective function may be discovered -- a proposal reified herein. We present \textbf{S}olution \textbf{A}nd \textbf{F}itness \textbf{E}volution (\textbf{SAFE}), a \textit{commensalistic} coevolutionary algorithm that maintains two coevolving populations: a population of candidate solutions and a population of candidate objective functions. As proof of principle of this concept, we show that SAFE successfully evolves not only solutions within a robotic maze domain, but also the objective functions needed to measure solution quality during evolution.

==> FuncOpt.tex <==
\section{Results: Function Optimization}
We chose three functions from the CEC 2015 competition involving real-parameter, single-objective optimization \cite{Liang2014}:

\begin{enumerate}
\item Rastrigin's Function:
\begin{equation}
\sum_{i=1}^{D}(x_i^2-10\cos(2 \pi x_i)+10)
\end{equation}

\item Rosenbrock's Function:
\begin{equation}
\sum_{i=1}^{D-1}(100(x_i^2-x_{i+1})^2 + (x_i-1)^2)
\end{equation}

\item  Cigar Function:
\begin{equation}
x_1^2 + 10^6\sum_{i=2}^{D}x_i^2 
\end{equation}
\end{enumerate}

$x_i \in [-100,100]$.
The global optimum is $0$ for all three functions.


\begin{table}
\centering
\caption{Function optimization results.}\label{tab:func}
\footnotesize
\begin{tabular}{|l|c|l|l|}
\hline
Function & Dimension & Algorithm & Average (SD) \\
\hline
Rastrigin & 2 & Standard EA & 0.019 (0.024) \\
Rastrigin & 2 & Novelty     & 5.609 (2.762) \\
Rastrigin & 2 & SAFE        & 0.020 (0.029) \\
Rastrigin & 2 & Random      & 3.523 (1.723) \\
\hline
Rastrigin & 10 & Standard EA & 2.021 (0.923) \\
Rastrigin & 10 & Novelty     &  1245.461 (356.491) \\
Rastrigin & 10 & SAFE        & 2.265 (0.896) \\
Rastrigin & 10 & Random      & 3201.528 (627.612) \\
\hline
Rastrigin & 20 & Standard EA & 11.304 (2.534) \\
Rastrigin & 20 & Novelty     & 6421.843 (1735.523) \\
Rastrigin & 20 & SAFE        &  11.316 (2.380) \\
Rastrigin & 20 & Random      & 17211.701 (2000.298) \\
\hline
Rosenbrock & 2 & Standard EA & 8.4259 (12.263) \\
Rosenbrock & 2 & Novelty     &  5.660 (5.4298) \\
Rosenbrock & 2 & SAFE        &  5.338 (9.308) \\
Rosenbrock & 2 & Random      & 1.344 (1.1879) \\
\hline
Rosenbrock & 10 & Standard EA & 166.748 (754.451) \\
Rosenbrock & 10 & Novelty     & 139121503 (91140685) \\
Rosenbrock & 10 & SAFE        &  67.107 (54.601) \\
Rosenbrock & 10 & Random      &  123240482 (52147119) \\
\hline
Rosenbrock & 20 & Standard EA &  472.520 (1281.838) \\
Rosenbrock & 20 & Novelty     & 1591371878 (562961244) \\
Rosenbrock & 20 & SAFE        & 363.582 (1123.496) \\
Rosenbrock & 20 & Random      &  2977485806 (706904757) \\
\hline
Cigar & 2 & Standard EA & 39.525 (86.082) \\
Cigar & 2 & Novelty     & 464.677 (554.321) \\
Cigar & 2 & SAFE        & 54.601 (111.112) \\
Cigar & 2 & Random      & 109.383 (105.872) \\
\hline
Cigar & 10 & Standard EA &  11521.859 (6992.152) \\
Cigar & 10 & Novelty     & 833329567 (310004729) \\
Cigar & 10 & SAFE        & 13397.482 (11054.069) \\
Cigar & 10 & Random      & 2233904549 (551030786) \\
\hline
Cigar & 20 & Standard EA & 141577.750 (68118.944) \\
Cigar & 20 & Novelty     & 5840943113 (1692212682) \\
Cigar & 20 & SAFE        & 152430.947 (62446.061) \\
Cigar & 20 & Random      & 15907463849 (2000417849) \\
\hline
\end{tabular}
\normalsize
\end{table}
